Efficient Robotic Policy Learning via Latent Space Backward Planning

Current robotic planning methods often rely on predicting multi-frame images with full pixel details. While this fine-grained approach can serve as a generic world model, it introduces two significant challenges for downstream policy learning: substantial computational costs that hinder real-time deployment, and accumulated inaccuracies that can mislead action extraction. Planning with coarse-grained subgoals partially alleviates efficiency issues. However, their forward planning schemes can still result in off-task predictions due to accumulation errors, leading to misalignment with long-term goals. This raises a critical question: Can robotic planning be both efficient and accurate enough for real-time control in long-horizon, multi-stage tasks? To address this, we propose a Latent Space Backward Planning scheme (LBP), which begins by grounding the task into final latent goals, followed by recursively predicting intermediate subgoals closer to the current state. The grounded final goal enables backward subgoal planning to always remain aware of task completion, facilitating on-task prediction along the entire planning horizon. The subgoal-conditioned policy incorporates a learnable token to summarize the subgoal sequences and determines how each subgoal guides action extraction. Through extensive simulation and real-robot long-horizon experiments, we show that LBP outperforms existing fine-grained and forward planning methods, achieving SOTA performance. Project Page: https://lbp-authors.github.io

==> icml2024/tables/algo.tex <==
\begin{algorithm}
    \caption{Pseudocode of the Proposed UAGLNet}
    \label{alg:UAGLNet}
    \renewcommand{\algorithmicrequire}{\textbf{Input: }}
    \renewcommand{\algorithmicensure}{\textbf{Output: }}
    \algorithmicrequire Input image $\mathbf{I}$; Ground truth mask $\mathbf{Y}$;\\
    \algorithmicensure Segmentation output $\mathbf{S}$; Local uncertainty $\mathbf{U}_{L}$; Global uncertainty $\mathbf{U}_{G}$;
    % Algorithm content goes here
    \begin{algorithmic}[1]
        \STATE //* \textit{Training Procedure} *//
        \FOR{\textit{Epochs}}{
            \FOR{\textit{Batches}}{
            \STATE//* \textit{Generate Hierarchical Features via CE} *//
            \STATE $\mathbf{F}_{1} \xleftarrow{\mathrm{MKFN}\times \mathrm{N}_{1}} I$
            \STATE $\mathbf{F}_{2} \xleftarrow{\mathrm{MKFN}\times \mathrm{N}_{2}} \mathbf{F}_{1}$
            \STATE $\mathbf{F}_{3} \xleftarrow{ \; \mathrm{CIB}\times \mathrm{N}_{3} \; } \mathbf{F}_{2}$
            \STATE $\mathbf{F}_{4} \xleftarrow{\mathrm{MHSA}\times \mathrm{N}_{4}} \mathbf{F}_{3}$
          
            \STATE//* \textit{Global-Local Fusion via GLF} *//
            \STATE $\mathbf{F}_{L} \xleftarrow{GLF} {\mathbf{F}_{1}, \mathbf{F}_{2}, \mathbf{F}_{3}}$
            \STATE $\mathbf{F}_{G} \xleftarrow{GLF} {\mathbf{F}_{3}, \mathbf{F}_{4}}$

            \STATE//* \textit{Mitigate Segmentation Ambiguity via UAD} *//
            \STATE $\bm{\mu}, \bm{\sigma} \leftarrow$ use $\Phi(\mathbf{F}_{L})$ to predict corresponding distribution 
            \STATE $\mathbf{x}^{(1)}, \mathbf{x}^{(2)}, ... ,\mathbf{x}^{(T)} \leftarrow$ randomly draw $T$ sample from $\mathcal{N}(\bm{\mu},\bm{\sigma}^2)$
            \STATE $\textbf{U}_{L} \leftarrow$ use $\mathrm{Norm}(\mathrm{Var}(\mathbf{x}^{(1)}, \mathbf{x}^{(2)}, ... ,\mathbf{x}^{(T)})$ to calculate local uncertainty map
            \STATE $U_{G} \leftarrow$  calculate global uncertainty map from $\mathbf{F}_{G}$ using the same method
            \STATE $\mathbf{F}_{out} \leftarrow (1 - \mathbf{U}_{G}) \times \mathbf{F}_{G} + (1-\mathbf{U}_{L}) \times \mathbf{F}_{L}$

            \STATE//* \textit{Obtain Final Segmentation and Compute Loss} *//
            \STATE $\mathbf{S} \leftarrow \mathbf{F}_{out}$
            \STATE $\mathcal{L}_{\mathrm{seg}}(\mathbf{S}) \leftarrow$ use $\mathbf{S}$ and $\mathbf{Y}$ to compute segmentation loss
            \STATE $\mathbf{x}^{(*)} \leftarrow$ randomly draw a sample from $\mathcal{N}(\bm{\mu},\bm{\sigma}^2)$
            \STATE $\mathcal{L}_{\mathrm{unc}}(\mathbf{U}_{L}) \leftarrow$ use $\mathbf{x}^{(*)}$ and $\mathbf{Y}$ to compute local uncertainty loss
            \STATE $\mathcal{L}_{\mathrm{unc}}(\mathbf{U}_{G}) \leftarrow$ compute global uncertainty loss from $\mathbf{F}_{G}$ using the same method
            \STATE $\mathcal{L}_{\mathrm{total}} \leftarrow \mathcal{L}_{\mathrm{seg}}(\mathbf{S}) + \lambda_{1} \mathcal{L}_{\mathrm{unc}}(\mathbf{U}_{G}) + \lambda_{2} \mathcal{L}_{\mathrm{unc}}(\mathbf{U}_{L})$
            \STATE Minimize $\mathcal{L}_{\mathrm{total}}$ and update the model parameters accordingly
            
            }\ENDFOR
        }\ENDFOR
        \STATE //* \textit{Testing Procedure} *// 
        \STATE Predict segmentation maps using UAGLNet
    \end{algorithmic}
\end{algorithm}
